Tracking Urbanization in Developing Regions with Remote Sensing Spatial-Temporal Super-Resolution

Automated tracking of urban development in areas where construction information is not available became possible with recent advancements in machine learning and remote sensing. Unfortunately, these solutions perform best on high-resolution imagery, which is expensive to acquire and infrequently available, making it difficult to scale over long time spans and across large geographies. In this work, we propose a pipeline that leverages a single high-resolution image and a time series of publicly available low-resolution images to generate accurate high-resolution time series for object tracking in urban construction. Our method achieves significant improvement in comparison to baselines using single image super-resolution, and can assist in extending the accessibility and scalability of building construction tracking across the developing world.

==> checklist.tex <==
\newpage
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See Section~\ref{intro}.}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{experiment},~\ref{impact}, Appendix G.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Section~\ref{impact}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{Yes.}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See Section~\ref{experiment} and Appendix B.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section 5 and Appendix B.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See Section~\ref{experiment}.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix B.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See Section~\ref{experiment}.}
  \item Did you mention the license of the assets?
    \answerYes{See Appendix C.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{See Section~\ref{experiment}, Appendix C.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{See Appendix C.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{See Appendix D.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerYes{See Appendix D.}
\end{enumerate}

\end{enumerate}

==> impact.tex <==
\section{Statement of Broader Impact}
\label{impact}

With our proposed Spatial-Temporal Super-Resolution approach, we aim to move the needle towards a more equitable social and economic environment in two ways. First, we hope that the ability to extend the availability of high resolution satellite imagery in areas where such images are temporally sparse will help narrow the data gap between regions of varying economic development and aid in decision making. On this point, we acknowledge that certain areas of the globe may still have no high resolution satellite coverage \cite{reid_2020}, in which case our approach may exacerbate the data gap by only helping regions that already have some high resolution satellite imagery. Second, we hypothesize that the presence of a high resolution temporally divergent conditional input along with the low resolution input at the desired time may help mitigate the impact of training set distribution bias. However, additional experiments are needed to evaluate this hypothesis, and our model is still expected to suffer from bias if trained on data that is not representative of the target distribution. Additionally, we acknowledge that increasing the temporal availability of high resolution satellite imagery has potential applications in surveillance. Finally, while we hope our approach can aid in large-scale downstream applications such as post-disaster building damage estimation and poverty prediction, we caution against using generated images to inform individual policy decisions (e.g. retroactively applying permit fees for swimming pools).

==> setup.tex <==
\subsection{Problem Setup}


